Learning Instance-Specific Augmentations by Capturing Local Invariances

We introduce InstaAug, a method for automatically learning input-specific augmentations from data. Previous methods for learning augmentations have typically assumed independence between the original input and the transformation applied to that input. This can be highly restrictive, as the invariances we hope our augmentation will capture are themselves often highly input dependent. InstaAug instead introduces a learnable invariance module that maps from inputs to tailored transformation parameters, allowing local invariances to be captured. This can be simultaneously trained alongside the downstream model in a fully end-to-end manner, or separately learned for a pre-trained model. We empirically demonstrate that InstaAug learns meaningful input-dependent augmentations for a wide range of transformation classes, which in turn provides better performance on both supervised and self-supervised tasks.

==> 110proof.tex <==
% \setcounter{theorem}{0}
% \begin{theorem}
% Let $p_{\psi}(z)$ and $q_{\phi,\psi}(z|x)$ represent respectively the pushforward distributions of $\mathcal{N}(0,I)$ and $q_{\phi}(y|x)$ along $g_{\psi}$. If $g_\psi$ is an invertible function, then
% \begin{align}
%     \ELBO_{\Y}(x,\theta,\phi,\psi) = 
%     \E_{q_{\phi,\psi}(z|x)} [\log p_{\theta}(x|z)]-\KL{q_{\phi,\psi}(z|x)}{p_{\psi}(z)}.
%     \label{eqn:appendix:1}
% \end{align}
% \end{theorem}
\maintheorem*
\begin{proof}

%%% refrences
% data processing inequality proof based on generalized log sum inequality:% https://web.stanford.edu/class/stats311/lecture-notes.pdf
% generalized log sum inequalityhttps://arxiv.org/pdf/2005.03272.pdf
% DPI proof http://www.stat.yale.edu/~yw562/teaching/598/lec04.pdf
% DPI result https://ocw.mit.edu/courses/electrical-engineering-and-computer-science/6-441-information-theory-spring-2016/lecture-notes/MIT6_441S16_course_notes.pdf
% degenerate conditonal Jensen https://math.stackexchange.com/questions/1643216/equality-in-conditional-jensens-inequality
% direct proof https://math.stackexchange.com/questions/4216714/why-does-relative-entropy-decrease-under-pushforward/4216773#4216773
% related proof https://www.math.univ-toulouse.fr/~agarivie/sites/default/files/3_KL_PAC.pdf

We first prove the inequality from \cref{eq:bound_on_KL}, then we show that \cref{eq:bound_on_KL} is actually an equality when $g_{\psi}$ is invertible, and finally we prove that the reconstruction term is unchanged by $g_{\psi}$.
% then that $\ELBO_{\Y}(x,\theta,\phi,\psi)$ equals $\ELBO_{\Z}(x,\theta,\phi,\psi)$ if $g_{\psi}$ is invertible. \\

% that the reconstruction and KL terms from \cref{eqn:appendix:2} are equal to the ones from~\cref{eq:bound_on_KL}.
%To deal with the situation where $\Z$ is a Euclidean space, and we cannot use Lebesgue measure on $\Z$, we define a new measure $\nu$ on $\Z$.

%where the second equation follows from the the definition of pushforward probability and  substituting $z=g_{\psi}(y)$.

% For the KL-terms, we first observe that for any measurable set $B\in \Y$,
% %\emile{better to use $p$ instead of $\mathcal{N}$}
% %\emile{I think there is a confusion between measures and densities: \url{https://en.wikipedia.org/wiki/Kullback-Leibler_divergence}}
% \begin{align}
% \begin{split}
%     q_{\phi}(y\in B|x)&=\int_{B} q_{\phi}(y|x)d\xi=\int_{B} \frac{q_{\phi}(y|x)}{p(y)}p(y)d\xi\\
%       &=\int_{g_{\psi}(B)} \frac{q_{\phi}(g_{\psi}^{-1}(z)|x)}{p(g_{\psi}^{-1}(z))}p_{\psi}(z)d\nu,
% \end{split}
% \end{align}
% %\begin{align}
% %\begin{split}
% %    q_{\phi}(y\in B|x)&=\int_{B} \frac{dq_{\phi}(y|x)}{d\mathcal{N}(y; 0, I)}d\mathcal{N}(y; 0, I)\\
% %      &=\int_{B} \frac{dq_{\phi}(y|x)}{d\mathcal{N}(y; 0, I)}dp_{\psi}(g_{\psi}(y))\\
% %      &=\int_{g_{\psi}(B)} \frac{dq_{\phi}(g_{\psi}^{-1}(z)|x)}{d\mathcal{N}(g_{\psi}^{-1}(z); 0, I)}dp_{\psi}(z).
% %\end{split}
% %\end{align}
% according to the Radon–Nikodym theorem, and
% \begin{align}
%     q_{\phi, \psi}(z\in g_\psi(B)|x)=\int_{g_{\psi}(B)} \frac{q_{\phi,\psi}(z|x)}{p_{\psi}(z)}p_{\psi}(z)d\nu.
% \end{align}
% Because $q_{\phi}(y\in B|x)=q_{\phi,\psi}(z\in g_\psi(B)|x)$ for any measurable set $B$, 
% \begin{align}
%     \frac{q_{\phi}(g_{\psi}^{-1}(z)|x)}{p(g_{\psi})}=\frac{q_{\phi,\psi}(z|x)}{p_{\psi}(z)}
% \end{align}
% holds almost everywhere.

% By the definition of KL-divergence,
% \begin{align}
% \begin{split}
%     \KL{q_{\phi}(y|x)}{p(y)}&=\E_{q_{\phi}(y|x)} \left[\log \frac{q_{\phi}(y|x)}{p(y)}\right]\\
%     &=\E_{q_{\phi, \psi}(z|x)}\left[\log \frac{q_{\phi}(g_{\psi}^{-1}(z)|x)}{p(g_{\psi}^{-1}(z))}\right]\\
%     &=\E_{q_{\phi, \psi}(z|x)}\left[\log \frac{q_{\phi,\psi}(z|x)}{p_{\psi}(z)}\right]\\
%     &=\KL{q_{\phi,\psi}(z|x)}{p_{\psi}(z)},
% \end{split}
% \end{align}
% which concludes the proof.

Let us denote by $\mathcal{F}$ and $\mathcal{G}$ the sigma-algebras of respectively $\Y$ and $\Z$, and we have by construction a measurable map $g_{\psi}: (\Y, \mathcal{F}) \rightarrow (\Z, \mathcal{G})$.
We can actually define the measurable space $(\Z, \mathcal{G})$ as the image of $(\Y, \mathcal{F})$ by $g_{\psi}$, then $g_{\psi}$ is automatically both surjective and measurable.\footnote{We recall that $g_{\psi}$ is said to be measurable if and only if for any $A \in \mathcal{G}$, $g_{\psi}^{-1}(A) \in \mathcal{F}$.}
% , where $A \in \mathcal{G}$, is measurable with respect to $\nu$ 
%  is measurable on $\Y$
We also assume that there exists a measure on $\Y$, which we denote $\xi$, and denote with $\nu$ the corresponding pushforward measure by $g_{\psi}$ on $\Z$.
We further have $\nu(A)=\xi(g_{\psi}^{-1}(A))$ for any $A \in \mathcal{G}$.\footnote{The notation $g_{\psi}^{-1}(A)$ does not imply that $g_{\psi}$ is invertible, but denotes the preimage of $A$ which is defined as $g_{\psi}^{-1}(A)=\{y \in \Y ~|~ g_{\psi}(y) \in A \}$.}

%
We start by proving \cref{eq:bound_on_KL}, where the Kullback-Leibler (KL) divergence between the two pushforward measures\footnote{We denote the pushforward of a probability measure $\chi$ along a map $g$ by $\chi \circ g^{-1}$.} 
$q_{\phi,\psi} \triangleq q_{\phi} \circ g_{\psi}^{-1}$ and $p_{\psi} \triangleq p \circ g_{\psi}^{-1}$ 
% $q_{\phi,\psi}(\cdot|x) \triangleq g_{\psi} \# q_{\phi}(\cdot|x)$ and $p_{\psi} \triangleq g_{\psi} \# p$ 
is upper bounded by $\KL{q_{\phi}(y|x)}{p(y)}$, where here we have $p(y)=\mathcal{N}(y;0,I)$ but we will use $p$ as a convenient shorthand.
At a high-level, we essentially have that \cref{eq:bound_on_KL} follows directly the data processing inequality \citep{sason2019DataProcessing} with a deterministic kernel $z=g_{\psi}(y)$.
%
% the KL divergence between $q_{\phi}(\cdot|x)$ and $p(\cdot)$.
Nonetheless, we develop in what follows a proof which additionally gives sufficient conditions for when this inequality becomes non-strict.
% To simplify the notation, we sometimes use 
We can assume that $\KL{q_{\phi}(y|x)}{\mathcal{N}(y; 0, I)}$ is finite, as otherwise the result is trivially true, which in turn implies $q_{\phi} \ll p$.\footnote{We denote the absolute continuity of measures with $\ll$, where $\mu$ is said to be absolutely continuous w.r.t.\ $\nu$, i.e.\ $\mu \ll \nu$, if for any measurable set $A$, $\nu(A)=0$ implies $\mu(A)=0$.}
%We first note that the KL divergence of interest is defined, i.e.\ $q_{\phi,\psi} \ll p_{\psi}$, since we assumed that .
For any $A \in \mathcal{G}$, we have that if 
$p_{\psi}(A) = p \circ g_{\psi}^{-1}(A) = p(g_{\psi}^{-1}(A)) = 0$ then this implies $q_{\phi}(g_{\psi}^{-1}(A)) = q_{\phi} \circ g_{\psi}^{-1}(A) = q_{\phi, \psi}(A) = 0$.
As such, we have that $q_{\phi,\psi} \ll p_{\psi}$ and so the $\KL{q_{\phi,\psi}(z|x)}{p_{\psi}(z)}$ is also defined.

Our next significant step is to show that
\begin{align} \label{eq:lemma}
\E_{p(y)} \left[\frac{q_{\phi}}{p} \given[\Big] \sigma(g_{\psi}) \right] = \frac{q_{\phi} \circ g_{\psi}^{-1}}{p \circ g_{\psi}^{-1}} \circ g_{\psi},
\end{align}
where $\sigma(g_{\psi})$ denotes the sigma-algebra generated by the function $g_{\psi}$.
To do this, let $h : (\Z, \mathcal{G}) \rightarrow (\R_+, \mathcal{B}(\R_+))$ be a measurable function s.t.\ $\E_{p(y)} \left[\frac{q_{\phi}}{p} \given[\Big] \sigma(g_{\psi}) \right] = h \circ g_{\psi}$. 
To show this, we will demonstrate that they lead to equivalent measures when integrated over any arbitrary set $A \in \mathcal{G}$:
%
\begin{align*} 
%\begin{split}
   \int_{\Z} \mathds{1}_{A} ~\frac{q_{\phi} \circ g_{\psi}^{-1}}{p \circ g_{\psi}^{-1}} ~ p \circ g_{\psi}^{-1} ~d\nu
   &= \int_{\Z} \mathds{1}_{A} ~q_{\phi} \circ g_{\psi}^{-1} ~d\nu %\\
   = \int_{\Z} \mathds{1}_{A} ~d(q_{\phi} \circ g_{\psi}^{-1}) \\
   &\stackrel{(a)}{=} \int_{\Y} (\mathds{1}_{A} \circ g_{\psi}) ~dq_{\phi} % ~d\xi \\
   = \int_{\Y} (\mathds{1}_{A} \circ g_{\psi}) ~q_{\phi} ~d\xi \\
   &\stackrel{(b)}{=} \int_{\Y} (\mathds{1}_{A} \circ g_{\psi}) ~\frac{q_{\phi}}{p} ~p ~d\xi \\
   &\stackrel{(c)}{=} \int_{\Y} (\mathds{1}_{A} \circ g_{\psi}) ~\E_{p(y)} \left[\frac{q_{\phi}}{p} \given[\Big] \sigma(g_{\psi}) \right] ~p ~d\xi \\
   &\stackrel{(d)}{=} \int_{\Y} (\mathds{1}_{A} \circ g_{\psi}) ~(h \circ g_{\psi}) ~p ~d\xi % \\
   = \int_{\Y} (\mathds{1}_{A} \circ g_{\psi}) ~(h \circ g_{\psi}) ~dp \\
   \displaybreak[0]
   &\stackrel{(e)}{=} \int_{\Z} \mathds{1}_{A} ~h ~d(p \circ g_{\psi}^{-1}) % \\
   = \int_{\Z} \mathds{1}_{A} ~h ~(p \circ g_{\psi}^{-1}) ~d\nu,
%\end{split}
\end{align*}
where we have leveraged the definition of pushforward measures in (a \& e); the absolute continuity of $q_{\phi}$ w.r.t.\ $p$ in (b); the conditional expectation definition in (c); and the definition of $h$ in (d).
By equating terms, we have that $q_{\phi} \circ g_{\psi}^{-1} / p \circ g_{\psi}^{-1} = h$, almost-surely with respect to $q_{\phi} \circ g_{\psi}^{-1}$ and thus that \cref{eq:lemma} is verified.

Let us define $f: x \mapsto x \log(x)$, which is strictly convex on $[0, \infty)$ (as it can be prolonged with $f(0)=0$).
We have the following
\begin{align*}
%\begin{split}
    \KL{q_{\phi,\psi}(z|x)}{p_{\psi}(z)}
    % &\stackrel{(a)}{=}\E_{q_{\phi,\psi}(z|x)} \left[\log\left(\frac{q_{\phi,\psi}}{p_{\psi}} (z) \right)\right] \\
    % &\stackrel{(c)}{=}\E_{p(y)} \left[f\left(\frac{q_{\phi,\psi}}{p_{\psi}} \circ g_{\psi}(y) \right)\right]\\
    % &\stackrel{(b)}{=}\E_{p_{\psi}(z)} \left[f\left(\frac{q_{\phi,\psi}}{p_{\psi}} (z) \right)\right] \\
    % &\stackrel{(d)}{=}\E_{p(y)} \left[f\left( \E_{p(y)} \left[\frac{q_{\phi}}{p} \given[\Big] \sigma(g_{\psi}) \right] \right)\right]\\
    % &\stackrel{(e)}{\le} \E_{p(y)} \left[ \E_{p(y)} \left[ f\left(\frac{q_{\phi}}{p}\right) \given[\Big] \sigma(g_{\psi}) \right] \right] \\
    % &\stackrel{(f)}{=}\E_{p(y)} \left[ f \left( \frac{q_{\phi}(y|x)}{p(y)} \right) \right] \\
    &\stackrel{(a)}{=} \int_{\Z} \log\left(\frac{q_{\phi,\psi}}{p_{\psi}} \right) q_{\phi,\psi} ~d\nu \\
    &\stackrel{(b)}{=} \int_{\Z} \log\left(\frac{q_{\phi,\psi}}{p_{\psi}} \right) \frac{q_{\phi,\psi}}{p_{\psi}} ~p_{\psi} ~d\nu \\
    &\stackrel{(c)}{=} \int_{\Z} f \left(\frac{q_{\phi,\psi}}{p_{\psi}} \right) ~p_{\psi}~ d\nu % \\
    = \int_{\Z} f \left(\frac{q_{\phi,\psi}}{p_{\psi}} \right) ~d(p \circ g_{\psi}^{-1}) \\
    &\stackrel{(d)}{=} \int_{\Y} f \left(\frac{q_{\phi,\psi}}{p_{\psi}} \circ g_{\psi} \right) ~dp% \\
    % = \int_{\Y} f \left(\frac{q_{\phi,\psi}}{p_{\psi}} \circ g_{\psi} \right) p ~d\xi \\
    \stackrel{}{=} \int_{\Y} f \left(\frac{q_{\phi} \circ g_{\psi}^{-1}}{p \circ g_{\psi}^{-1}} \circ g_{\psi} \right) p ~d\xi \\
    &\stackrel{(e)}{=} \int_{\Y} f\left( \E_{p(y)} \left[\frac{q_{\phi}}{p} \given[\Big] \sigma(g_{\psi}) \right] \right) p ~d\xi\\
    &\stackrel{(f)}{\le} \int_{\Y} \E_{p(y)} \left[ f\left(\frac{q_{\phi}}{p}\right) \given[\Big] \sigma(g_{\psi}) \right] p ~d\xi \\ 
    &\stackrel{(g)}{=} \int_{\Y} f \left( \frac{q_{\phi}}{p} \right) p ~d\xi \\
    &\stackrel{(h)}{=} \int_{\Y} \log \left( \frac{q_{\phi}}{p} \right) \frac{q_{\phi}}{p} ~p ~d\xi \\
    &\stackrel{(i)}{=}\E_{q_{\phi}(y|x)} \left[\log \left(\frac{q_{\phi}(y|x)}{p(y)} \right) \right] \\
    &\stackrel{(j)}{=}\KL{q_{\phi}(y|x)}{p(y)},
%\end{split}
\end{align*}
where we leveraged the definition of the KL divergence in (a \& j); the absolute continuity of $q_{\phi}$ w.r.t.\ $p$ in (b \& i); the definition of $f$ in (c \& h); the definition of the pushforward measure in (d); \cref{eq:lemma} in (e); the conditional Jensen inequality in (f) and the law of total expectation in (g).
Note that this proof not only holds for the KL divergence, but for any f-divergences as they are defined as in (b) with $f$ convex.

To prove \cref{eq:elbo_equivalence}, we now need to show that line (f) above becomes an equality when $g_{\psi}$ is invertible.
%we still need to study the conditions for which the conditional Jensen inequality in (e) is not strict, i.e.\ where it is an equality.
As $f$ is strictly convex, this happens if and only if $\frac{q_{\phi}}{p} = \E_{p(y)} \left[\frac{q_{\phi}}{p} \given[\Big] \sigma(g_{\psi}) \right]$.
A sufficient condition for this to be true is for $\frac{q_{\phi}}{p}$ to be measurable w.r.t.\ $\sigma(g_{\psi})$ which is satisfied when $g_{\psi}: \Y \mapsto \Z$ is invertible as $\sigma(g_{\psi}) \supseteq \mathcal{F}$, as required.
We have thus shown that the KL divergences are equal when using an invertible $g_{\psi}$.
% contains all open sets from $\Y$. 
%

% We now show that the reconstruction terms from $\ELBO_{\Y}(x,\theta,\phi,\psi)$ and $\ELBO_{\Z}(x,\theta,\phi,\psi)$ are equal where by definition we have
% \begin{align}
%     \ELBO_{\Y}(x,\theta,\phi,\psi) \triangleq \E_{q_{\phi}(y|x)} [\log p_{\theta}(x|g_{\psi}(y))] 
%         - \KL{q_{\phi}(y|x)}{p(y)},
%     \label{eqn:appendix:2}
% \end{align}
% with $p(y)=\mathcal{N}(y; 0, I)$ being a standard normal distribution.

% According to the definition of pushforward probabilities $p_{\psi}(z)$ and $q_{\phi,\psi}(z|x)$,
% %\begin{align}
% %    \int_{\Y} \mathds{1}_{g_{\psi}^{-1}(A)}(g_{\psi}(y)) p(y)d\xi &=\int_{\Z} \mathds{1}_{A}(z) p_{\psi}(z)d\nu,\\
% %    \int_{\Y} \mathds{1}_{g_{\psi}^{-1}(A)}(g_{\psi}(y)) q_{\phi}(y|x)d\xi &=\int_{\Z} \mathds{1}_{A}(z) q_{\phi,\psi}(z|x)d\nu.
% %\end{align}
% %And consequently,
% \begin{align}
%     \int_{\Y} f(g_{\psi}(y)) p(y)d\xi &=\int_{\Z} f(z) p_{\psi}(z)d\nu,\\
%     \int_{\Y} f(g_{\psi}(y)) q_{\phi}(y|x)d\xi &=\int_{\Z} f(z) q_{\phi,\psi}(z|x)d\nu.
% \end{align}
% for any measurable function $f$.

For the reconstruction term, we instead have
\begin{align*}
%\begin{split}
    \E_{q_{\phi}(y|x)} [\log p_{\theta}(x|g_{\psi}(y))]
    &=\int_{\Y} \log p_{\theta}(x|g_{\psi}(y)) q_{\phi}(y|x)d\xi\\
    &=\int_{\Z} \log p_{\theta}(x|z) q_{\phi,\psi}(z|x)d\nu\\
    &=\E_{q_{\phi,\psi}(z|x)} [\log p_{\theta}(x|z)].
%\end{split}
\end{align*}
%
\cref{eq:elbo_equivalence} now follows from the fact that both the reconstruction and KL terms are equal.
%we have that $\ELBO_{\Y}(x,\theta,\phi,\psi) = \ELBO_{\Z}(x,\theta,\phi,\psi)$.


\end{proof}


%To give the criteria for high-quality decoders which maps Gaussian prior~$\mathcal{N}(0,1)$ to MoG data distribution~$\frac{1}{2}\mathcal{N}(-\mu,\sigma)+\frac{1}{2}\mathcal{N}(\mu,\sigma)$, we need to make the following definitions. To make sure that the two components of MoG is separated, we assume $\mu \le 4\sigma$.

%We first define two closed intervals $X^0= [-\mu-3\sigma, -\mu+3\sigma]$ and $X^1 = [\mu-3\sigma, \mu+3\sigma]$ as the high density intervals, and $X^C=(X^0\cup X^1)^C$ as the low density area with $P_X(X^C) \le 0.003$. We further define $Z^i$ and $Z^C$ as disjoint pre-images of $X^i$ and $X^C$ under decoding for $i=0,1$. 
%To ensure that the push forward distribution decoder$(P_Z)$ matches $P_X$ well, the following two criteria must be satisfied.
%\begin{align}
%    &P_Z(Z^C) \le \epsilon,\label{eqn:criterion_1}\\
%    &\frac{1}{1+\epsilon} \le \frac{P_Z(Z^0)}{P_Z(Z^1)} \le 1+\epsilon,\label{eqn:criterion_2}
%\end{align}
%\begin{itemize}
%    \item $P_Z(Z^C) < \epsilon$,
%    \item $1-\epsilon \le \frac{P_Z(Z^0)}{P_Z(Z^1)} \le 1+\epsilon$,
%\end{itemize}
%where $\epsilon$ is a small positive value. The first criterion limits the proportion of samples from $P_Z$ which are decoded to low density area $X^C$. The second criterion ensures the balance of generated samples in $X^0$ and $X^1$. 

%Then we can write the main theorem as follows.
%\begin{theorem}
%    To ensure the decoder satisfies the conditions in Eqn.~\ref{eqn:criterion_1} and \ref{eqn:criterion_2} with error bound $\epsilon$, 
%    the Lipschitz constant of the decoder $L\ge \frac{2\mu-6\sigma}{d(\epsilon)}$, where $d(\epsilon)$ is a monotone decreasing function of $\epsilon$ shown in Eqn.~\ref{eqn:d}.
%\end{theorem}

%To prove the main theorem, we need the following lemmas.
%\begin{lemma}
%    \label{lemma:1}
%    If the two criteria are satisfied, $P_Z(Z^i) \ge \frac{1}{2}-\epsilon$, for $i=0,1$. 
%\end{lemma}
%\begin{proof}
%    Combining Eqn.~\ref{eqn:criterion_1} and Eqn.~ \ref{eqn:criterion_2}, we get
%    \begin{align}
%        P_Z(Z^i)+(1+\epsilon)P_Z(Z^i)&\ge 1-P_Z(Z^C)\ge 1-\epsilon,\\
%        P_Z(Z^i)&\ge \frac{1-\epsilon}{2+\epsilon}\ge \frac{1}{2}-\epsilon,
%    \end{align}
%    for both $i=0,1$.
%\end{proof}

%\begin{lemma}
%    \label{lemma:1}
%    We define $a=$min($\{l\le 0$, where $[-l, l]$ intersects with both $Z^0$ and $Z^1)\})$. 
%    As long as Eqn.~\ref{eqn:criterion_1} and \ref{eqn:criterion_2} are satisfied,
%    $a \le \Phi ^{-1}(0.75+\epsilon)$, where $\Phi ^{-1}$ is the inverse c.d.f. of standard Gaussian distribution.
%\end{lemma}
%\begin{proof}
%    For convenience, we define interval $I=[-\Phi ^{-1}(0.75+\epsilon), \Phi ^{-1}(0.75+\epsilon)]$.
%    If $a > \Phi ^{-1}(0.75+\epsilon)$, for $i_0=0$ or $1$, $Z^{i_0} \cap I =\o$ and $Z^{i_0} \subseteq I^C$.  Then
%    \begin{align}
%        P_Z(Z^{i_0}) \le P_Z(I^C) = \frac{1}{2}-2\epsilon,
%    \end{align} which violates Lemma~\ref{lemma:1}.
%\end{proof}

%As a result, $Z^0$ and $Z^1$ both intersect with $I$. Now we can move on to the main theorem.
%\begin{proof}
%     To start with, we define $d$ as the distance between $Z^0\cap I$ and $Z^1\cap I$ and find the closest point pair 
%     \begin{align}
%         (z^0, z^1) = \mathop{\arg\min}_{z^0, z^1} |z^0-z^1|,
%     \end{align}
%     for $z^0\in Z^0\cap I$ and $z^1\in Z^1\cap I$. 
%     Assuming without loss of generality that $z^0 \le z^1$, it's easy to know that $[z^0, z^1]\in Z^C$. Then 
%     \begin{align}
%         P_Z(Z^C) \ge P_Z([z^0, z^1]) \ge d\phi(\Phi ^{-1}(0.75+\epsilon)),
%     \end{align} 
%     where $\phi$ is the p.d.f of standard Gaussian distribution.
%     Due to Eqn.~\ref{eqn:criterion_1}, we can derive that that 
%     \begin{align}
%         d(\epsilon) < \frac{\epsilon}{\phi(\Phi ^{-1}(0.75+\epsilon))}.\label{eqn:d}
%     \end{align}
%     In the meanwhile, because $z^0\in Z^0$ and $z^1\in Z^1$, 
%     \begin{align}
%         |\text{decode}(z^0)-\text{decode}(z^1)| \ge 2\mu-6\sigma.
%     \end{align}
%     So the Lipschitz constant of the decoder 
%     \begin{align}
%         L\ge \frac{|\text{decode}(z^0)-\text{decode}(z^0)|}{|z^0-z^1|} \ge \frac{2\mu-6\sigma}{d(\epsilon)}.
%     \end{align}
%\end{proof}
%Since $d(\epsilon)$ is very small, for small postive $\epsilon$, $L$ is usually very large. For example, when $\epsilon=1\%$, $d(\epsilon)=0.03$, and $L>150$ for $\mu=3$ and $\sigma=0.5$.

==> old_comments.tex <==
title and abstract
%\ning{Tom said: I would avoid having a name that is so tied into Augerino as you are then placing all our utility on their work.  If we are going to name it like this, we have to frame the whole thing as an Augerino extension from start to finish and have our motivation be fully based on them.  I don't think we really want that so should avoid a name like this. } %\adam{Is that the InstAug name :( ?}

intro.tex
\yann{I would not talk about group equivarant network. Everyone uses augmentations and know they are useful, we have to convince readers that  current augmentations are not good enough.
I would do (1) data augmentation used everywhere; (2) augmentations are not instance independent which can give issues as in Fig 1; (3) challenge is that having a human saying what augmentations to use for all instance is not scalable; (4) we learn them from training data; (5) its better.}
\ning{Re: I think we should start from a bigger problem, because we are actually learning some invariance, rather than only improving data augmentation.}
\emile{Need to give more credit to Augerino / more background on how it works. Perhaps should rename `global augmentation' to `Augerino' or `Augerino-like'?}
\ning{I will introduce Augerino more. But the global augmentation is not the same as Augerino in cropping. Augerino cannot do cropping. But in color jittering we can rename `global augmentation' to `Augerino'}
\hyunjik{I think we can make section 2 be titled Related work \& background, where we introduce Augerino as background, moving some of the material from the current section 3.3 to this section. This will set the stage for the paper and also give more credit to Augerino as the source of inspiration of our work.}

\ning{We need to change notations. (1) tranformation, (2) target label, (3) task}

\hyunjik{I like Yann's suggestion of kicking off the intro with augmentations, because then the paper feels much more relevant for the broader DL community compared to when we're starting with invariance, since as Yann says augmentations are super widely used whereas invariance (although closely related to augmentations) is not something at the forefront of most people's minds in DL. This is also more consistent with the title of the paper. However I do think that we should mention invariance \& group invariant/equivariant networks further into the intro, as it's definitely relevant work. One way we could do this is by the following variation on Yann's suggestion, which can be mostly acheived by reordering the content we already have: (1) Data augmentation is used everywhere (2) Data augmentation broadly has two effects - regularization \& incorporating invariance. (3) Invariance should be instance dependent but currently it isn't, so we can get issues like Fig 1 or the leaf/lime example (4) human labelling of invariances per data point is not scalable (5) Using invariant/equivariant NNs does not solve this issue either since they also assume global invariance + mention difficulties of making them expressive hence they are less widely used. (6) Hence we propose to learn instance specific aug from training data. (7) We show that it works better on tasks x,y,z.}
\ning{I personally feel it would be better to start the paper with invariance, rather than directly talk about augmentations. Firstly, I'd love to locate our problem in a broader topic of invariance, which I think is more interesting than data augmentation. In fact, we can learn at least some part of the invariance, which is quite meaningful. I don't want to regard these results as intermediate products in pursuit of higher performance.
Meanwhile, we don't want readers to feel that our goal is to improve base model performance by proposing a novel augmentation method. 
If so, we have to beat other strong augmentation methods, which are actually orthogonal to \method .}
\hyunjik{Here's how I think about this: researchers who specialize in group equivariant NNs will share your view that invariance is the 'broader topic' than augmentation because they see data augmentation as one particular way of achieving invariance, and so they might be more drawn into the paper if we start off with invariance. But from the perspective of most other DL researchers/practioners, data augmentation is not only a way for achieving invariance, but it's also a regularization method, and arguably the effect of regularization is much more powerful than that of invariance. The reason they care about augmentation is not because it gives you invariance, but because it just works so well for boosting performance in many contexts (supervised learning, self-supervised learning etc). So from their perspective, invariance is the narrower and less interesting topic. So I'd argue that people would think your paper is much more relevant and broader scope if you introduce it with data augmentation rather than invariance. The paper is really about tackling shortcoming of augmentation methods from the perspective of invariance, and I think starting the paper with data augmentation doesn't make the paper feel incremental or merely a new augmentation method. We can always emphasise the invariance aspect later on in the intro as I'm suggesting. Also another reason I'm against making the paper sound as too much of an invariance paper is that we have no quantitative metrics for measuring how good our learned invariances are, and only have qualitative results.}
\ning{I agree. I will move the first paragraph to related work and elaborate more on augmentations.}
%(Importance of invariance and how it is used)
\yann{what is the use of invariance whcih you find broader than augmentation  Ning?  interpretability ? data understanding ? if it's more than performance / sample efficiency then we should probably test those and mention those in the motivation.
}
\adam{To add my two cents: I would start with augmentation. Augmentation is the thing everyone does, it's on the surface. Then get into why they do it---relates to invariance. Also, augment is in our title so...}
\emile{We can indeed introduce the notion of invariance at the end of the intro as a way to formalise what it means to learn (instance specific) 'good augmentations'?}

%\adam{Perhaps one or two lines at the start---what is the problem? Problem is data scarcity, lack of generalization, all the general criticisms that people level at deep learning. }

%\adam{Again, maybe lead in with a more general problem---supposing we want to do augmentation to solve aforementined data scarcity problems, we need to choose concretely the augmentation transformations to apply. How do we do that / what assumptions are we encoding by choosing them? This just sets up the text below, which I think is good.}
%\adam{In between these, we could mention Augerino. For example, most prior work is completely heuristic about the augmentations. Augerino and a few others decided to try and \emph{learn} the augmentation. But there remains the assumption that augmentations should apply independently to different instances. This motivates...}
%\hyunjik{What follows in this paragraph is way too much detail for the intro. We should just mention that there is a module that takes data as input and outputs the augmentation distribution and we learn this with an appropriate loss that's detailed in Sec 3. The rest should be in Sec 3 or 2 if we choose to talk about Augerino in sec 2.}

related.tex
%\hyunjik{we should also include related work on learning invariances here. Some that I can think of now: Meta-Learning Symmetries by Reparameterization, Automatic Symmetry Discovery with Lie Algebra Convolutional Network}


method.tex
%\adam{just wondering, so we need $\T$ here? Could we not simply have a distribution $p(y, \x)$. Also confusing that $t$ and $\T$ are completely unrelated.}
\hyunjik{It might be better to use a different name for the parameter module, since `parameters' can be confused with the parameters of a neural net, whereas here these are referring to the parameters of the augmentation distribution. We can just call it a (learned/neural) augmentation module}

\hyunjik{Again here it might be more intuitive to replace the red circle and blue square in Fig4 with patches of cows/grass, with different patches at different positions on the plane of the decision boundary. Not sure if it can be done in a way that's neat, but think it's worth thinking about as this point on training signal is an important point to make clear.}
\ning{I can't agree more. Do you guys have any idea how to do it?}

For simpler transformations with uniform distributions, we follow Augerino to simply use the volume of the distribution's support set to measure diversity. For example, we have two parameters $\theta_{\min}$ and $\theta_{\max}$ to parameterize rotation, then $div(P_{\theta})=|\theta_{\max}-\theta_{\min}|$
For more complicated localized transformations, we use entropy instead, where the diversity metric is defined as $\mathbb{H}[t|\x] \triangleq \mathbb{E}_t [-\log(p_{\theta}(t|\x))]$ for each $\x$. \emile{div is confusing, isn't this simply the entropy?}
\yann{Can we put all in a single framework: Div is always max entropy. As special case  for simple parameters we use uniform distribution which gives $\implies |\theta_{\max}-\theta_{\min}|$. Right now it seems we treat those aug differently.}
\emile{isn't the entropy $\log(\theta_{\max}-\theta_{\min})$ for the continuous distribution?}
\ning{Yes, the difference is the log. We are trying to using the same way to evaluate diversity as Augerio}
\hyunjik{It's fine to put everything in the same framework first (i.e. use entropy and so use $\log(\theta_{\max}-\theta_{\min})$) then mention that in practice we remove the log.}

\adam{Perhaps move this equation way earlier, or at least its intuitive explanation earlier. Basically we want to trade off model performance and augmentation diversity. That is like \emph{the} key idea of how to train InstAug. We can they break down what the components actually mean.}


%\yann{I think this section has too many low level details before even knowing what we'll end up optimizing. In general I think we should spend more time early on motivating / formalizing the higher level idea / goal of the method}
%\adam{Yes, move loss function up, give general description of InstAug, then explain how we concretely deal with crops, colours and so on.}

%\yann{this paragraph could be extended by giving example / figure  ? Although  simple and intuitive, most people don't know augerino. It's important they get the simple ones before moving to complicated augmentations .}

\adam{This is all very Augerino-centric, assuming that their way is the right way. We should just focus on describing our own ideas and explaining why it is in general good. It is surprising that we need a $H_{\max}$, so worth just explaining that idea from first principles.}

experiment.tex

in the example figure
\emile{Row 4 isn't very vegetarian friendly.}
 \ning{Row 4 is aimed to show the multi-modality distribution, It's not easy to find a figure with such property. But we can certainly remove or replace it.}
  \emile{Could be useful to add quantitative metric to assess the learned distribution of croppings; Could be the variance of the center of the crops (the more concentrated, the better?).}
  \ning{I don't think there is a proper metric to directly assess the distributions of cropping. Smaller variance of centers does not mean good cropping because we are also encouraging diversity, let along the multi-modality shown in row 4.}
  
  
%\hyunjik{We should also mention why we don't use a continuous reparameterizable distribution for crops e.g. parameterising dsitribution over centre, height and width of crop. Was the reason because this underperformed compared to the current approach?} \ning{discuss: yes. We tried that, doesn't work very well. We should mention it as a failed attempt?}

\emile{That's the standard procedure for this dataset? if so state it.} \ning{There isn't a standard procedure for this task because people use the dataset in different ways.}

 %\hyunjik{minor: I think we need to make it clearer that theta is the parameters for the transformation distrib rather than NN parameters of the controller. Maybe use separate params for these $\theta, \phi$ and introduce the $\phi$ as what we're minimizing in Eq 1. Currently Eq 1\&2 looks as if we're optimizing wrt $\theta$, which isn't what we're doing. It might be more natural to swap $\theta$ and $\phi$ in this case, just because $\theta$ usually refers to the params of a NN.}
 
 %\ning{Is it ok if we remove 'which is motivated by Augerino'?} \hyunjik{In fact I think we should mention Augerino at the very beginning of the section, and say that the loss function is adapted from the loss proposed in Augerino. This section is where it's most relevant, so we should give it fair credit.}
% \emile{}
%\emile{Likely worth mentioning the concept of maximum invariant cf Yann.}
%\adam{I don't really understand Fig 3, we should spend a bit of time making a pretty and explanatory visual, as this is kind of the first thing people will look at.}

%\adam{Is this formula right? I would have thought we are doing $\mathbb{E}_{\x \sim p_{\text{data}}}~[\mathbb{H}[ p_{\phi{(\x)}}(\tau(\x))]]$. This one can be estimated unbiasedly from batches, the other one cannot.}
%\yann{I agree with Adam, it seems natural to use the conditional entropy $\mathbb{H}[\Tilde{X}|X]$ than the marginal $\mathbb{H}[\Tilde{X}]$ (also easier to understand from fig 3). }

%\hyunjik{Need to make it clearer what this is. We should probably first say entropy is how we measure diversity, and that the entropy of the transformed samples is intractable after writing out this entropy in maths.} 
% \adam{I agree with Hyunjik's commented out point. I think skipping straight to $\mathbb{H}[ p_{\phi{(\x;\theta)}}(\tau)]$ makes it easier on the reader.}

==> preamble/acronyms.tex <==
\glsdisablehyper{}

\newacronym{KL}{KL}{Kullback-Leibler}
\newacronym{ELBO}{elbo}{\emph{evidence lower bound}}
\newacronym{MCMC}{mcmc}{Markov chain Monte Carlo}

\newacronym{ML}{ML}{machine learning}
\newacronym{VAE}{VAE}{variational auto-encoder}
\newacronym{VAETV}{VAE-TV}{variational auto-encoder with twin hidden variables}
\newacronym{AE}{AE}{auto-encoder}
\newacronym{SGD}{SGD}{stochastic gradient descent}
\newacronym[sort=beta]{BVAE}{\(\beta\)-vae}{}
\newacronym{TC}{TC}{total correlation}
\newacronym{DGM}{DGM}{deep generative model}
\newacronym{MMD}{MMD}{maximum mean discrepancy}
\newacronym{GAN}{GAN}{generative adversarial network}
\newacronym{AAE}{AAE}{adversarial auto-encoder}
\newacronym{CCM}{CCM}{constant curvature manifold}
\newacronym{IWAE}{IWAE}{importance weighted auto-encoder}
\newacronym{MC}{MC}{Monte Carlo}
\newacronym{NN}{NN}{neural network}
\newacronym{FNN}{FNN}{feedforward neural network}
\newacronym{MLP}{MLP}{multilayer perceptron}
\newacronym{SVM}{SVM}{support vector machine}
\newacronym{KDE}{KDE}{kernel density estimation}
\newacronym{RKHS}{RKHS}{reproducing kernel Hilbert space}
\newacronym{VI}{VI}{variational inference}
\newacronym{maxlike}{ML}{maximum likelihood}

==> preamble/preamble.tex <==
\usepackage
[acronym,smallcaps,nowarn,section,nogroupskip,nonumberlist]{glossaries}
\glsdisablehyper{}
